Noise-Assisted Variational Quantum Thermalization

Preparing thermal states on a quantum computer can have a variety of applications, from simulating many-body quantum systems to training machine learning models. Variational circuits have been proposed for this task on near-term quantum computers, but several challenges remain, such as finding a scalable cost-function, avoiding the need of purification, and mitigating noise effects. We propose a new algorithm for thermal state preparation that tackles those three challenges by exploiting the noise of quantum circuits. We consider a variational architecture containing a depolarizing channel after each unitary layer, with the ability to directly control the level of noise. We derive a closed-form approximation for the free-energy of such circuit and use it as a cost function for our variational algorithm. By evaluating our method on a variety of Hamiltonians and system sizes, we find several systems for which the thermal state can be approximated with a high fidelity. However, we also show that the ability for our algorithm to learn the thermal state strongly depends on the temperature: while a high fidelity can be obtained for high and low temperatures, we identify a specific range for which the problem becomes more challenging. We hope that this first study on noise-assisted thermal state preparation will inspire future research on exploiting noise in variational algorithms.

==> buffer.tex <==
\section{Related work}

Using variational circuits to prepare a thermal state presents two challenges specific to this task: 1) finding an ansatz that can prepare mixed states, 2) finding a scalable optimization strategy.

\subsection{Ansatz choice}

\paragraph{Purification ansatz} A common approach to thermal state preparation consists in preparing a purification of the thermal state using a variational circuit that acts on $2n$ qubits---$n$ system qubits and $n$ ancilla qubits---, and tracing the ancilla qubits out at the end of the circuit \cite{hsieh-variational-tfd,nasa-thermal-state,ibm-imaginary-time, entropy-taylor}. An example of purification often considered in the literature is the thermofield double (TFD) state \cite{hsieh-variational-tfd,nasa-thermal-state}. For a Hamiltonian $H$ and an inverse temperature $\beta$, it is given by
\begin{align} \label{eq:tfd}
    \ket{\text{TFD}}=\frac{1}{\sqrt{Z}} \sum_n e^{-\beta E_n / 2} \ket{n}_S \otimes \ket{n}_E
\end{align}
where the $\{E_n, \ket{n}\}_n$ are pairs of eigenvalue/eigenvector of $H$, and $Z=\Tr\left[e^{-\beta H}\right]$. Tracing out the environment directly gives the thermal state:
\begin{align*}
    \begin{split}
        \Tr_E[\ketbra{TFD}] &= \frac{1}{Z} \sum_n e^{-\beta E_n} \ket{n}_S \\
        &= \frac{1}{Z} e^{-\beta H}
    \end{split}
\end{align*}
For instance, \cite{hsieh-variational-tfd} and \cite{nasa-thermal-state} use a QAOA ansatz acting on $2n$ qubits to prepare the TFD state of the TFIM, the Ising chain, the XY chain, and free fermions. One advantage of this approach is the ability to simulate the TFD, which can be interesting in in its own right, for instance for studying black-holes \cite{thermofield-double}. The obvious disadvantage is that it requires twice as many qubits that the thermal state we want to simulate.

\paragraph{Initial mixed state} A converse approach consists in starting with a mixed state $\rho_0$ and applying a unitary ansatz on the $n$ qubits of the system. $\rho_0$ can either be fixed \cite{verdon2017quantum} or modified during the optimization process \cite{product-spectrum-ansatz,verdon2019quantum}.
In \cite{verdon2017quantum}, $\rho_0$ is the fixed thermal state of $H_I=\sum_{i=1}^n Z_i$, which can be easily prepared using the following purification:
\begin{align}
    \bigotimes_j \sqrt{2 \cosh(\beta)} \sum_{b \in \{0,1\}^n} e^{(-1)^{1+b} \beta / 2} \ket{b}_S \ket{b}_{E}
\end{align}
However, since the spectrum does not change when we apply the unitary ansatz, having a static $\rho_0$ fixes the spectrum of the final state. Therefore, if the spectrum of the thermal state we want to approximate is far from the spectrum of $\rho_0$, this approach will fail.
In \cite{product-spectrum-ansatz}, $\rho_0(\bm{\epsilon})$ is the thermal state of $H=\sum_{i=1}^n \epsilon_i P_i$, where $P_i=\frac{1-Z_i}{2}$ and $\bm{\epsilon}=\{\epsilon_1,...,\epsilon_n \}$ are parameters optimized during the training process:
\begin{align}
    \rho_0(\bm{\epsilon})=\bigotimes_{i=1}^n \frac{e^{-\beta \epsilon_i P_i}}{1+e^{-\beta \epsilon_i}}
\end{align}
Finally, \cite{verdon2019quantum} proposes to use a unitary with stochastic parameters to prepare $\rho_0$. More precisely,
\begin{align}
    \rho_0(\bm{\theta})=V(X_{\bm{\theta}})\ketbra{0} V(X_{\bm{\theta}})^\dag
\end{align}
where $V(\bm{x})$ is a unitary ansatz and $X_{\bm{\theta}} \sim p_{\bm{\theta}}$ is a random vector with parametrized density $p_{\bm{\theta}}$. The density $p_{\bm{\theta}}$ can be given by a classical model, such as an energy-based model (e.g. restricted Boltzmann machine) or a normalizing flow, which will be trained to get a $\rho_0$ with a spectrum close to the thermal state we want to approximate.

\subsection{Optimization strategies}

Once we have the ansatz, we need to optimize it. Two approaches have been proposed in the literature: 1) explicitly minimizing the free energy, 2) using imaginary-time evolution.

\paragraph{Free energy methods}
As shown in the Appendix (todo), the thermal state is the density matrix that minimizes the free energy. Therefore, in the same way as VQE uses the energy as a cost function, any thermal state preparation method can use the free energy as a cost function \cite{hsieh-variational-tfd,nasa-thermal-state,verdon2017quantum,verdon2019quantum}. However, one main difference with VQE is that the free energy cannot be easily estimated. Indeed, the Von Neumann entropy term, as a non-linear function of $\rho$, cannot be turned into an observable, and doing a full quantum state tomography would be very costly. Several methods have been proposed to solve this challenge:
\begin{itemize}
    \item Computing several Renyi entropies $S_{\alpha}=\frac{1}{1-\alpha} \Tr\left[ \rho^{\alpha} \right]$ (using multiple copies of $\rho$) and approximating the Von Neumann entropy with them \cite{hsieh-variational-tfd}
    \item Computing the entropies locally on a small subsystem \cite{hsieh-variational-tfd}
    \item Approximate the Von Neumann entropy by truncating its Taylor \cite{entropy-taylor} or Fourier \cite{wiebe-entropy-fourier} decomposition.
\end{itemize}

\paragraph{Imaginary-time evolution} Thermal state preparation be seen as the application of imaginary-time evolution during a time $\Delta t=i\beta/2$ on the maximally-mixed state $\rho_m=\frac{1}{d} \id$:
\begin{align*}
    \rho_{\beta}=\left( \frac{1}{C} e^{-\beta H/2} \right) \left( \frac{1}{d} \id \right) \left(\frac{1}{C}e^{-\beta H/2}\right)
\end{align*}
It's possible to simulate imaginary-time evolution using a variational circuit \cite{imaginary-time-evolution-benjamin} using a specific update rule. In \cite{ibm-imaginary-time}, the authors use a variational circuit $U(\thetab)$ on $2n$ qubits, initialized such that
\begin{align*}
    U(\thetab_0) \ket{0}^{\otimes 2n} \approx \ket{\Phi^+}
\end{align*}
where $\Phi^+$ is a maximally-entangled state. An imaginary-time update rule with a small learning rate $\tau$ will lead to a unitary $U(\thetab_0)$ such that:
\begin{align*}
    U(\thetab_1) \ket{0}^{\otimes 2n} \approx \frac{1}{C} e^{-\tau H} \ket{\Phi^+}
\end{align*}
Repeating it during $k=\frac{\beta}{2}$ steps will give the state
\begin{align*}
    U(\thetab_k) \ket{0}^{\otimes 2n} \approx \frac{1}{C} e^{-\beta H / 2} \ket{\Phi^+}
\end{align*}
whose trace on the environment is the thermal state. In \cite{japanese-imaginary-time}, the authors also use imaginary-time evolution to prepare the thermal state, but manage to reduce the number of qubits to $n$ when the Hamiltonian is diagonal in the $Z$-basis.
